Karma: Resource Allocation for Dynamic Demands

We consider the problem of fair resource allocation in a system where user demands are dynamic, that is, where user demands vary over time. Our key observation is that the classical max-min fairness algorithm for resource allocation provides many desirable properties (e.g., Pareto efficiency, strategy-proofness, and fairness), but only under the strong assumption of user demands being static over time. For the realistic case of dynamic user demands, the max-min fairness algorithm loses one or more of these properties. We present Karma, a new resource allocation mechanism for dynamic user demands. The key technical contribution in Karma is a credit-based resource allocation algorithm: in each quantum, users donate their unused resources and are assigned credits when other users borrow these resources; Karma carefully orchestrates the exchange of credits across users (based on their instantaneous demands, donated resources and borrowed resources), and performs prioritized resource allocation based on users' credits. We theoretically establish Karma guarantees related to Pareto efficiency, strategy-proofness, and fairness for dynamic user demands. Empirical evaluations over production workloads show that these properties translate well into practice: Karma is able to reduce disparity in performance across users to a bare minimum while maintaining Pareto-optimal system-wide performance.

==> banal <==
#!/usr/bin/perl -s
#
# Copyright (C) 2007 Geoffrey M. Voelker
#
# banal -- analyze pdf formatting 
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.
#
# Geoffrey M. Voelker (voelker@cs.ucsd.edu)
#

# todo:
# -- computer modern roman fonts
# -- embedded java script, remoteapproach.com

use Data::Dumper;
use File::Basename;

sub usage {
    print <<EOF
usage: banal [-report | -stats | -judge [specs]] [-zoom=N] files

banal has three modes of operation:

-report  print full formatting info for all pages.  this mode is
	 the default if no mode is specified:

         % banal paper.pdf

-stats   print formatting info condensed into one line with fields
         separated by tabs; useful for computing summary stats across
         many papers.

         fields are 'file', 'paper', 'text region', 'margins', 'font', 
         'leading', 'columns', 'pages', 'app'.  for example:

         % banal -stats *.pdf | cut -f 5 

         extracts font sizes from a set of pdf files.

-judge   compare document formatting against a set of formatting
         specifications:

         -paper=type     paper type ('letter' and 'A4' currently supported)
         -pages=num      max number of pages
         -font=num       min font size
	 -leading=num    min leading
         -cols=num       max columns
         -width=inches   max text region width
         -height=inches  max text region height
         -fudge=inches   text region fudge factor (helps with latex
			 overflow; default is $banal_text_fudge inches)

         specifications can consist of any and all elements in any
         combination.  for example:
         
         % banal -judge -paper=letter -pages=14 -font=10 -leading=12 -width=6.5 -height=9 *.pdf

         will check whether a set of pdf files conforms to formatting specs
         that require 8.5" x 11" paper, max 14 pages, min 10 point font,
	 min 12 point leading, and a max text region of 6.5" x 9".

         -format=lines|list

         lines   report format violations on multiple lines (default)

         list    report format violations on a single line separated by a
                 comma (e.g., for importing into a spreadsheet).

         % banal -judge -format=list [specs] *.pdf

  -   -   -   -   -   -   -   -   -   -   -   -   -   -   -   -   -   -

-zoom=N   passed to pdftohtml.  -zoom=1 means do not pass a zoom argument,
          and use pdftohtml\'s default zoom.

-version  report the version of banal

EOF
}

# version
$banal_version = "1.2.2";

# zoom value
usage() if ((defined $zoom) && ($zoom !~ /^[1-9]\d*(\.\d*)?$/));

# mapping from pdftohtml units to inches
#$p2h_per_inch = 72;
$p2h_per_inch;

# scale factor from pdftohtml units to points
#$p2h_to_points = 72 / $p2h_per_inch;
$p2h_to_points;

# minimum amount of text on page for it to be interesting
$banal_min_density = 8000;

# fudge factor when judging text regions (in inches).
$banal_text_fudge = 0.05;

# minimum number of pages that have to fail the text region specs.
# often papers have 1-2 pages where text on a table or figure extends
# into the margin.  when judging an entire paper, we'll let those slide...
$banal_judge_min_fail_pages = 3;

# policy to use to estimate leading
$banal_leading_policy;

# pdftohtml executable
if (exists $ENV{"PDFTOHTML"}) {
    $pdftohtml = $ENV{"PDFTOHTML"};
} elsif (exists $ENV{"PHP_PDFTOHTML"}) {
    $pdftohtml = $ENV{"PHP_PDFTOHTML"};
} elsif (defined $pdftohtml_prog) {
    $pdftohtml = $pdftohtml_prog;
} else {
    $pdftohtml = "pdftohtml";
}

#print STDERR "using $pdftohtml...\n";

# version of pdftohtml program
$p2h_version = 0;

# full path of file being analyzed
$banal_fullpath = '';
# file name of file being analyzed
$banal_filename = '';

# sketch of perl data structures used
$page = "
$num
$pagedata
$pagespec
";

$pagedata = "


";

$pagespec = "
$paperbb
$regionbb
$bodyfont
$ncols
";


$bbox = "
$top
$left
$width
$height
";

$segdata = "
%widths
%lefts
%rights
%tops
%bots
%leads
";


# return min key in hash
sub minkey ($) {
    my ($href) = @_;
    return (sort { $a <=> $b } keys %$href)[0];
}

# return max key in hash
sub maxkey ($) {
    my ($href) = @_;
    return (sort { $a <=> $b } keys %$href)[$#_ - 1];
}

# return key of mode of values in hash
sub modevalkey ($) {
    my ($href) = @_;
    my ($mode) = (keys %$href)[0];
    map { $mode = $_ if ($href->{$_} > $href->{$mode}) } keys %$href;
    return $mode;
}

# return max val in hash
sub maxval ($) {
    my ($href) = @_;
    my ($max) = (keys %$href)[0];
    map { $max = $_ if ($href->{$_} > $href->{$max}) } keys %$href;
    return $href->{$max};
}

# return 'a' == 'b'
sub bb_equal ($$) {
    my ($a, $b) = @_;
    return (($a->{top} == $b->{top}) &&
	    ($a->{left} == $b->{left}) &&
	    ($a->{height} == $b->{height}) &&
	    ($a->{width} == $b->{width}));
}

# merge 'a' into 'b'
sub bb_merge ($$) {
    my ($a, $b) = @_;

    $b->{top} = $a->{top} if ($a->{top} < $b->{top});
    $b->{left} = $a->{left} if ($a->{left} < $b->{left});
    $b->{height} = $a->{height} if ($a->{height} > $b->{height});
    $b->{width} = $a->{width} if ($a->{width} > $b->{width});
}

sub calc_page_body_font ($) {
    my ($page) = @_;
    my ($mode) = modevalkey ($page->{pagedata}->{segdata}->{byfont});
    $page->{pagedata}->{bodyfont} = $page->{doc}->{fonts}->{$mode};
    $page->{pagespec}->{bodyfont} = p2h_font_to_font_size ($page->{pagedata}->{bodyfont});
    if ($page->{pagespec}->{bodyfont} == 0) {
	print "$banal_filename: Error: Zero font on page $page->{num}, font id $mode\n";
    }
}

sub utf8ascii_undo ($) {
    my ($str) = @_;

    return $str unless ($str =~ /^\\376\\377(\\\d\d\d.)*$/);

    # string is UTF-8 in ASCII (not binary)
    #   (PDFCreator seems to like to do this, also freepdfconvert)
    print "$banal_filename: ascii UTF-8: $title\n" if ($debug_docapp);

    $str =~ s/\\376\\377//;
    $str =~ s/\\000//g;

    print "$banal_filename: unencoded: $str\n" if ($debug_docapp);
    return $str;
}

sub utf8bin_undo ($) {
    my ($str) = @_;

    return $str unless ($str =~ /^\376\377(\000.)*$/);

    # string is UTF-8 in binary
    print "$banal_filename: bin UTF-8: $str\n" if ($debug_docapp);

    $str =~ s/\376\377//;
    $str =~ s/\000//g;

    print "$banal_filename: unencoded $str\n" if ($debug_docapp);
    return $str;
}

sub utf8revbin_undo ($) {
    my ($str) = @_;

    # bytes reversed: character then null bytes (ScanSoft on the Mac)

    return $str unless ($str =~ /^\377\376(.\000)*$/);

    # string is UTF-8 in binary
    print "$banal_filename: rev bin UTF-8: $str\n" if ($debug_docapp);

    $str =~ s/\377\376//;
    $str =~ s/\000//g;

    print "$banal_filename: unencoded $str\n" if ($debug_docapp);
    return $str;
}

sub utf8hex_undo ($) {
    my ($str) = @_;

    return $str unless ($str =~ /^FEFF(00..)*$/i);

    print "$banal_filename: hex UTF-8: $str\n" if ($debug_docapp);

    $str =~ s/^FEFF//i;
    $str =~ s/00//g;
    print "$banal_filename: hex ascii: $str\n" if ($debug_docapp);
    $str = pack ("H*", $str);

    print "$banal_filename: packed $str\n" if ($debug_docapp);
    return $str;
}

# inferring the document application has two steps:
#   1) extracting the doc metadata
#   2) mapping metadata info to an application
#
# for (1), ideally we could use a module or tool to extract the
# InfoDict from the end of the pdf file.  but there are some cases
# where we need to peek outside the InfoDict for additional hints, so
# in the end we still have to scan through the pdf file ourselves.
#
# for (2), the world would be a simpler place if applications followed
# some kind of convention.  but given the large combination of apps,
# pdf converters, and OSes, of course the world is not so simple.  so,
# as usual, it's back to heuristics gathered from samples...

sub calc_doc_app ($) {
    my ($doc) = @_;
    my ($fname) = $doc->{fullpath};

    my ($creator, $title, $producer, $creatortool, $ptex);
    my ($rdftitle, $pdfproducer);
    my ($indirect, $quartzpdf, $pdfmachine, $cmrfont, $texfont);

    $creator = $title = $producer = $creatortool = $ptex = '';
    $rdftitle = $pdfproducer =  '';
    $indirect = $quartzpdf = $pdfmachine = $cmrfont = $texfont = 0;

    my ($app, @allapps);
    $app = '';
    @allapps = ();

    if (!open (PDF, $fname)) {
	print STDERR "$banal_filename: Error: Failed to open $fname for inferring doc app.";
	$doc->{app} = 'unknown';
	return;
    }

    while (<PDF>) {

	if (m|\/Creator\s*\(([^\)]+)\)|) {
	    $creator = $1;
	} elsif (m|\/Creator\s*<([^\)]+)>|) {
	    # UTF-8 ascii hex
	    $creator = utf8hex_undo ($1);
	} elsif (m|\/Creator \d+ \d+ R|) {
	    # Indirection:
	    # << /Producer 313 0 R /Creator 314 0 R ...
	    $indirect = 1;
	}

	if (m|\/Title\s*\(([^\)]+)\)|) {
	    $title = $1;
	} elsif (m|\/Title\s*<([^\)]+)>|) {
	    # UTF-8 ascii hex
	    $title = utf8hex_undo ($1);
	} elsif (m|<dc:title>.+<rdf:li.+>(.+)</rdf:li>.+</dc:title>|) {
	    $rdftitle = $1;
	} elsif (m|<dc:title>|) {
	    unless (m|</dc:title>|) {
		while (<PDF>) {
		    last if (m|</dc:title>|);
		    next unless (m|<rdf:li.+>(.+)</rdf:li>|);
		    $rdftitle = $1;
		}
	    }
	}

	if (m|\/Producer\s*\(([^\)]+)\)|) {
	    $producer = $1;
	} elsif (m|\/Producer\s*<([^\)]+)>|) {
	    # UTF-8 ascii hex
	    $producer = utf8hex_undo ($1);
	} elsif (m|<pdf:Producer>(.+)</pdf:Producer>|) {
	    $pdfproducer = $1;
	}

	# xap: Adobe Extensible Authoring and Publishing (early name, 5.0)
	# xmp: Adobe Extensible Metadata Platform (final name)
	if (m|<x[am]p:CreatorTool>(.+)<\/x[am]p:CreatorTool>|) {
	    $creatortool = $1;
	}

	if (m|<pdfx:PTEX|) {
	    # <pdfx:PTEX.Fullbanner>This is pdfTeX...</pdfx:PTEX.Fullbanner>
	    $ptex = 1;
	}

	if (m|\(Mac OS.+Quartz PDFContext\)|) {
	    # (Mac OS X 10.6.2 Quartz PDFContext) [producer indirection]
	    $quartzpdf = 1;
	} elsif (m|\(TeX\)|) {
	    # (TeX) [creator indirection]
	    $tex = 1;
	} elsif (m|% created by pdfMachine|) {
	    # tool doesn't bother to create any metadata whatsoever...
	    $pdfmachine = 1;
	}

	if (!$cmrfont && m|(\/BaseFont\s*\/\w+\+[Cc][Mm][Rr]\d+)|) {
	    # /BaseFont/EGYAWT+CMR8
	    $pdf_tools{'cmr fonts'}++;
	    $cmrfont = 1;
	} elsif (!$texfont && m|/BaseFont\s*/\w+\+([Cc][Mm]\w\w\d+)|) {
	    $pdf_tools{'tex fonts'}++;
	    $texfont = $1;
	}

    }

    close (PDF);

    # undo any UTF-8 in ascii (literally "\376\377\000P\000r\000o...")
    $title = utf8ascii_undo ($title) if ($title);
    $creator = utf8ascii_undo ($creator) if ($creator);
    $producer = utf8ascii_undo ($producer) if ($producer);
    $creatortool = utf8ascii_undo ($creatortool) if ($creatortool);
    $rdftitle = utf8ascii_undo  ($rdftitle) if ($rdftitle);
    $pdfproducer = utf8ascii_undo ($pdfproducer) if ($pdfproducer);

    # undo any UTF-8 in binary
    $title = utf8bin_undo ($title) if ($title);
    $creator = utf8bin_undo ($creator) if ($creator);
    $producer = utf8bin_undo ($producer) if ($producer);
    $creatortool = utf8bin_undo ($creatortool) if ($creatortool);
    $rdftitle = utf8bin_undo  ($rdftitle) if ($rdftitle);
    $pdfproducer = utf8bin_undo ($pdfproducer) if ($pdfproducer);

    # undo any UTF-8 in binary (reversed)
    $title = utf8revbin_undo ($title) if ($title);
    $creator = utf8revbin_undo ($creator) if ($creator);
    $producer = utf8revbin_undo ($producer) if ($producer);
    $creatortool = utf8revbin_undo ($creatortool) if ($creatortool);
    $rdftitle = utf8revbin_undo  ($rdftitle) if ($rdftitle);
    $pdfproducer = utf8revbin_undo ($pdfproducer) if ($pdfproducer);

    $title = $rdftitle if (!$title && $rdftitle);

    # Word
    if ($creator =~ /Microsoft.+Word/) {
        # Mac OS Quartz PDFContext, doPDF
	$pdf_tools{'word in creator'}++;
	$app = 'word';
    } elsif ($title =~ /Microsoft Word \-/) {
        # ps->pdf w/ gs, distiller
	# often doc name in title after '-' (but not always)
	$pdf_tools{'gs, distiller'}++;
	$app = 'word';
    } elsif ($title =~ /Proceedings Template \- WORD/i) {
	$pdf_tools{'template'}++;
	$app = 'word';
    } elsif ($creator =~ /easyPDF/) {
        # BCL easyPDF
	$pdf_tools{'easyPDF'}++;
	$app = 'word';
    } elsif ($creator =~ /PDFCreator/) {
	$pdf_tools{'PDFCreator'}++;
	$app = 'word';
    } elsif ($creator =~ /PDFMaker.+Word/) {
	$pdf_tools{'PDFMaker'}++;
	$app = 'word';
    } elsif ($creator =~ /Sonic PDF/) {
	$pdf_tools{'sonic pdf'}++;
	$app = 'word';
    } elsif ($creatortool =~ /Word/) {
	# Adobe XMP metadata
	$pdf_tools{'Acrobat PDFMaker'}++;
	$app = 'word';
    } elsif ($producer =~ /freepdfconvert|deskPDF|ReportLab|PDF reDirect/) {
	$pdf_tools{'misc pdf tools'}++;
	$app = 'word';
#    } elsif ($creator =~ /\000M\000i\000c\000r\000o\000s\000o\000f\000t.+\000W\000o\000r\000d/i) {
	# UTF-8 binary
#	$pdf_tools{'Word (UTF-8)'}++;
#	$app = 'word';
    } elsif ($pdfmachine) {
	$pdf_tools{'pdfmachine'}++;
	$app = 'word';
    } elsif ($title =~ /\.docx?$/i) {
	# Amyuni puts the filename in the title
	$pdf_tools{'doc(x) extension'}++;
	$app = 'word';
    }

    if ($app) {
	push (@allapps, $app);
	$app = '';

	# never seen this happen, but let's sanity check...
	if ($cmrfont) {
	    print "$banal_filename: Warning: CMR font in Word doc?\n";
	    $pdf_tools{'** cmrfont in word doc'}++;
	}
    }
    
    # TeX
    if ($creator =~ /TeX/) {
	$pdf_tools{'tex in creator'}++;
	$app = 'tex';
    } elsif ($creatortool =~ /(MiK)?TeX/) {
	$pdf_tools{'(mik)tex in creatortool'}++;
	$app = 'tex';
    } elsif ($creator =~ /dvips/) {
	$pdf_tools{'dvips in creator'}++;
	$app = 'tex';
    } elsif ($producer =~ /dvips/) {
	$pdf_tools{'dvips in producer'}++;
	$app = 'tex';
    } elsif ($producer =~ /PrimoPDF/ && $title =~ /\.dvi$/) {
	$pdf_tools{'primopdf'}++;
	$app = 'tex';
    } elsif (($creator =~ /gnuplot/) && ($producer =~ /Ghostscript|Distiller/)) {
	# highly likely a tex document
	$pdf_tools{'gnuplot + gs|dist'}++;
	$app = 'tex';
    } elsif ($producer =~ /Ghostscript|PDFContext|pstopdf|AntennaHouse PDF/ && !$creator && !$title) {
	# just a producer tag, no other InfoDict metadata...
	# have yet to see a Word doc that didn't like InfoDict metadata
	$pdf_tools{'only producer'}++;
	$app = 'tex';
    } elsif ($indirect && $quartzpdf && $tex) {
	if ($creator || $producer) {
	    print "$banal_filename: Warning: direct and indirect InfoDict entries\n";
	}
	$pdf_tools{'tex quartzpdf'}++;
	$app = 'tex';
    } elsif ($creatortool =~ /gnuplot/ && !$creator && !$producer && !$title) {
	$pdf_tools{'only gnuplot'}++;
	$app = 'tex';
    } elsif ($ptex) {
	$pdf_tools{'pdftex in pdfx'}++;
	$app = 'tex';
    } elsif ($producer =~ /Ghostscript/ && $title =~ /\.pdf$/) {
	$pdf_tools{'gs ps to pdf'}++;
	$app = 'tex';
    } elsif ($cmrfont) {
	$pdf_tools{'cmrfont'}++;
	$app = 'tex';
    }

    if ($app) {
	push (@allapps, $app);
	$app = '';
    }

    # OpenOffice
    if ($producer =~ /OpenOffice/) {
	$pdf_tools{'open office'}++;
	push (@allapps, 'openoffice');
    }

    if ($creator =~ /Interleaf/) {
	$pdf_tools{'interleaf + distiller'}++;
	push (@allapps, 'interleaf');
    }

    # FrameMaker (!)
    if ($creator =~ /FrameMaker/) {
	$pdf_tools{'frame'}++;
	push (@allapps, 'framemaker');
    }

    # sanity check that we haven't matched more than one application,
    # or whether we didn't match anything...
    if (scalar (@allapps) > 1) {
	print STDERR "$banal_filename: Error: multiple apps inferred: @allapps\n";
	$app = 'unknown';
    } elsif (scalar (@allapps) < 1) {
	print STDERR "$banal_filename: Warning: failed to infer document app, using 'unknown'\n";
#	print STDERR "$banal_filename:   Creator: $creator\n" if ($creator);
#	print STDERR "$banal_filename:   Title: $title\n" if ($title);
#	print STDERR "$banal_filename:   Producer: $producer\n" if ($producer);
#	print STDERR "$banal_filename:   CreatorTool: $creatortool\n" if ($creatortool);
#	print STDERR "$banal_filename:   RDFTitle: $rdftitle\n" if ($rdftitle);
#	print STDERR "$banal_filename:   PDFProducer: $pdfproducer\n" if ($pdfproducer);
#	print STDERR "$banal_filename:   cmrfont\n" if ($cmrfont);
#	print STDERR "$banal_filename:   texfont $texfont\n" if ($texfont);
	$app = 'unknown';
    } else {
	$app = $allapps[0];
    }

#    $pdf_tools{$app}++;
    $doc->{app} = $app;

    if ($debug_docapp) {
	print STDERR "$banal_filename: Creator: $creator\n" if ($creator);
	print STDERR "$banal_filename: Title: $title\n" if ($title);
	print STDERR "$banal_filename: Producer: $producer\n" if ($producer);
	print STDERR "$banal_filename: CreatorTool: $creatortool\n" if ($creatortool);
	print STDERR "$banal_filename: RDFTitle: $rdftitle\n" if ($rdftitle);
	print STDERR "$banal_filename: PDFProducer: $pdfproducer\n" if ($pdfproducer);
	print STDERR "$banal_filename: cmrfont\n" if ($cmrfont);
	print STDERR "$banal_filename: texfont $texfont\n" if ($texfont);
	foreach $t (keys %pdf_tools) {
	    print "$t: $pdf_tools{$t}\n";
	}
    }

    return;
}

sub calc_page_leading ($) {
    my ($page) = @_;
#    my ($mode) = modevalkey ($page->{pagedata}->{segdata}->{leads});
    my ($mode, $segs);

    $segs = $page->{pagedata}->{segdata_byfont}->{$page->{pagedata}->{bodyfont}->{id}};
    $mode = modevalkey ($segs->{leads});

    $count = $segs->{leads}->{$mode} +
	$segs->{leads}->{$mode - 1} +
	$segs->{leads}->{$mode + 1};
    if ($count <= 0) {
	$page->{pagespec}->{lead} = 0;
	return;
    }

    if ($banal_leading_policy eq 'mode') {
	print "using leading policy 'mode'\n" if ($debug_leading);
	$lead = $mode * $p2h_to_points;
	$lead *= 10;
	$lead = int ($lead + 0.5);
	$lead /= 10;
	print "leading: $lead\n" if ($debug_leading);
	$page->{pagespec}->{lead} = $lead;
	return;
    }

    if ($debug_leading) {
        # leading histogram
	$ll = $segs->{leads};
	foreach $k (sort { $a <=> $b } keys %$ll) {
	    my ($l) = int (($k * $p2h_to_points * 10) + 0.5);
	    $l /= 10;
	    print "$l ($segs->{leads}->{$k}) ";
	}
	print "\n";
    }

    $wsum = $mode * ($segs->{leads}->{$mode} / $count);
    $wsum += ($mode - 1) * ($segs->{leads}->{$mode - 1} / $count);
    $wsum += ($mode + 1) * ($segs->{leads}->{$mode + 1} / $count);
    $lead = $wsum * $p2h_to_points;
    $lead *= 10;
    $lead = int ($lead + 0.5);
    $lead /= 10;

    $page->{pagespec}->{lead} = $lead;

#    print Dumper ($segs->{leads});
}

sub calc_page_columns ($) {
    my ($page) = @_;
    my ($pagew);
    my ($segs, $maxw, $colw, $ncols);

    # use estimated width of text region as base
    $pagew = $page->{pagespec}->{textbb}->{width};

    # use the maximum width segment in the body font to estimate
    # column width
    $segs = $page->{pagedata}->{segdata_byfont}->{$page->{pagedata}->{bodyfont}->{id}};
#    $maxw = maxkey ($segs->{widths});
    $modew = modevalkey ($segs->{widths});
    $colw = $modew / $p2h_per_inch;

    if ($colw >= ($pagew / 2.0)) {
	$ncols = 1;
    } elsif (($colw < ($pagew / 2.0)) && ($colw >= ($pagew / 3.0))) {
	$ncols = 2;
    } elsif (($colw < ($pagew / 3.0)) && ($colw >= ($pagew / 4.0))) {
	$ncols = 3;
    } elsif (($colw < ($pagew / 4.0)) && ($colw >= ($pagew / 5.0))) {
	$ncols = 4;
    } elsif (($colw < ($pagew / 5.0)) && ($colw >= ($pagew / 6.0))) {
	$ncols = 5;
    } elsif (($colw < ($pagew / 6.0)) && ($colw >= ($pagew / 7.0))) {
	$ncols = 6;
    } elsif (($colw < ($pagew / 7.0)) && ($colw >= ($pagew / 8.0))) {
	$ncols = 7;
    } elsif ($page->{pagespec}->{density} < $banal_min_density) {
	$ncols = 1;
    } else {
	my ($num) = $page->{num};
#	print Dumper ($segs->{widths});
	printf ("$banal_filename: Error (page $num): Unknown number of columns: width of typical text segment %.2fin, page %.2fin.\n", $colw, $pagew);
	$ncols = 1;
    }

    $page->{pagedata}->{ncols} = $ncols;
    $page->{pagespec}->{ncols} = $ncols;
}

sub calc_page_text_region ($$) {
    my ($page, $segdata) = @_;
    my ($minw, $maxw, $minh, $maxh);
    my ($segs_minw, $segs_maxw);

    $segs_minw = $segdata->{lefts};
    $segs_maxw = $segdata->{rights};

    # find the minimum left position among segments (must be
    # multiple segments with that position to skip outliers)
    $minw = 8 * $p2h_per_inch;

    foreach $s (keys %$segs_minw) {
	$minw = $s if (($s < $minw) && ($segs_minw->{$s} > 3));
    }

    # all consistency bets are off with low density pages 
    $minw = minkey ($segs_minw) if ($minw > 4 * $p2h_per_inch);

    # find the maximum right position among segments (must be
    # multiple segments with that position to skip outliers)
    $maxw = 0;
    foreach $s (keys %$segs_maxw) {
	$maxw = $s if (($s > $maxw) && ($segs_maxw->{$s} >= 2));
    }

#    print "tmpw $tmpw maxw $maxw\n";
#    if ($maxw < 600) {
#	print Dumper ($segs_maxw);
#    }

    # unjustified text may not have multiple segments with the same
    # max right position...fall back to just using the max right position
    $maxw = maxkey ($segs_maxw) if ($maxw < $minw);
    $maxw = $minw + minkey ($segdata->{widths}) if (!defined $maxw);
    $maxw = $minw if ($maxw < $minw);

    $minh = minkey ($segdata->{tops});
    $maxh = maxkey ($segdata->{bots});

    $page->{pagedata}->{textbb} = {
	top => $minh,
	left => $minw,
	width => ($maxw - $minw),
	height => ($maxh - $minh),
    };

#    print "$minw $maxw\n";
#    print Dumper ($page->{pagedata}->{textbb});

    $page->{pagespec}->{textbb} = {
	top => $minh / $p2h_per_inch,
	left => $minw / $p2h_per_inch,
	width => ($maxw - $minw) / $p2h_per_inch,
	height => ($maxh - $minh) / $p2h_per_inch,
    };

    return 1;
}

sub calc_page_density ($) {
    my ($page) = @_;
    my ($bfont, $density);

    $bfont = $page->{pagedata}->{bodyfont}->{id};
    $density = maxval ($page->{pagedata}->{segdata_byfont}->{$bfont}->{byfont});
    $page->{pagespec}->{density} = $density;
}

sub calc_doc_body_font ($) {
    my ($doc) = @_;
    my ($fonts) = {};

    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};
	$fonts->{$page->{pagespec}->{bodyfont}}++;
    }

    $doc->{pagespec}->{bodyfont} = modevalkey ($fonts);
}

sub calc_doc_leading ($) {
    my ($doc) = @_;
    my ($leads) = {};
    my ($lmode, $page);

    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};
	$leads->{$page->{pagespec}->{lead}}++;
    }
    $lmode = modevalkey ($leads);

#    $use_raw_leading = 1;
    if (!defined $use_raw_leading) {
#	print "mode: $lmode\n";
#	print "pages w mode: $leads->{$lmode}\n";
	if ($leads->{$lmode} >= $doc->{npages} / 2) {
	    for $i (1..$doc->{npages}) {
		$page = $doc->{pages}->{$i};
		next if ($page->{pagespec}->{lead} == $lmode);

#		print "abs diff: ", $lmode - $page->{pagespec}->{lead}, "\n";
		if (abs ($lmode - $page->{pagespec}->{lead}) < 0.2) {
#		    print "setting to ", $lmode, "\n";
		    $page->{pagespec}->{lead} = $lmode;
		}
	    }
	}
    }

    if ($debug_leading) {

	print "entire doc\n";

	for $i (1..$doc->{npages}) {
	    $page = $doc->{pages}->{$i};
	    $segs = $page->{pagedata}->{segdata_byfont}->{$page->{pagedata}->{bodyfont}->{id}};
	    $leads = $segs->{leads};
	    foreach $k (keys %$leads) {
		$doc_leads{$k} += $segs->{leads}->{$k};
		$lcount++;
	    }
	}

	foreach $k (sort { $a <=> $b } keys %doc_leads) {
	    my ($l) = int (($k * $p2h_to_points * 10) + 0.5);
	    $l /= 10;
	    print "$l ($doc_leads{$k}) ";
	}
	print "\n";

	{
	    $mode = modevalkey (\%doc_leads);
	    print "mvk $mode\n";
	    $count = $doc_leads{$mode} +
		$doc_leads{$mode - 1} +
		$doc_leads{$mode + 1};

	    $wsum = $mode * ($doc_leads{$mode} / $count);
	    print "b: ", $wsum, "\n";
	    $wsum += ($mode - 1) * ($doc_leads{$mode - 1} / $count);
	    $wsum += ($mode + 1) * ($doc_leads{$mode + 1} / $count);
	    $lead = $wsum * $p2h_to_points;
	    print "c: ", $lead, "\n";
	    $lead *= 10;
	    print "d: ", $lead, "\n";
	    $lead = int ($lead + 0.5);
	    $lead /= 10;
	    print "lead: $lead\n";
	}
    }

    $doc->{pagespec}->{lead} = $lmode;
}

sub calc_doc_text_region ($) {
    my ($doc) = @_;
    my ($page, $maxw, $maxh, $minl, $mint, $rmarg, $bmarg);

    $page = $doc->{pages}->{1};
    $maxw = $page->{pagespec}->{textbb}->{width};
    $maxh = $page->{pagespec}->{textbb}->{height};
    $minl = $page->{pagespec}->{textbb}->{left};
    $mint = $page->{pagespec}->{textbb}->{top};

    for $i (2..$doc->{npages}) {
	next if ($page->{density} < $banal_min_density);

	$page = $doc->{pages}->{$i};
	$maxw = $page->{pagespec}->{textbb}->{width} if
	    ($page->{pagespec}->{textbb}->{width} > $maxw);
	$maxh = $page->{pagespec}->{textbb}->{height} if
	    ($page->{pagespec}->{textbb}->{height} > $maxh);
	$minl = $page->{pagespec}->{textbb}->{left} if
	    ($page->{pagespec}->{textbb}->{left} < $minl);
	$mint = $page->{pagespec}->{textbb}->{top} if
	    ($page->{pagespec}->{textbb}->{top} < $mint);

    }
    $doc->{textbb}->{width} = $maxw;
    $doc->{textbb}->{height} = $maxh;
    $doc->{textbb}->{left} = $minl;
    $doc->{textbb}->{top} = $mint;

    $rmarg = $doc->{pagespec}->{paperbb}->{width} - ($doc->{textbb}->{width} + $doc->{textbb}->{left});
    $bmarg = $doc->{pagespec}->{paperbb}->{height} - ($doc->{textbb}->{height} + $doc->{textbb}->{top});
    if ($rmarg < 0) {
	print "r MARGIN\n";
    }
    if ($bmarg < 0) {
	print "b MARGIN\n";
    }
    $doc->{textbb}->{rmarg} = $rmarg;
    $doc->{textbb}->{bmarg} = $bmarg;
}

sub calc_doc_page_types ($) {
    my ($doc) = @_;
    my ($page, $font, $type);
    
    $font = $doc->{pagespec}->{bodyfont};

    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};
	$type = 'body';

	if ($i == 1 && $page->{pagespec}->{density} < 3000) {
	    $type = 'cover';
	} elsif ($page->{pagespec}->{bodyfont} < $font) {
	    if (($doc->{npages} - $i) < ($doc->{npages} / 3)) {
		$type = 'bib';
	    }
	} elsif ($page->{pagespec}->{density} < $banal_min_density) {
	    if ($i == $doc->{npages}) {
		$type = 'bib';
	    } else {
		$type = 'figure';
	    }
	}

	$page->{pagespec}->{type} = $type;
    }
}

sub calc_doc_columns ($) {
    my ($doc) = @_;
    my ($page);
    my ($cols) = {};

    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};
	$cols->{$page->{pagespec}->{ncols}}++;
    }

    # number of columns on greatest number of pages
    $doc->{ncols} = modevalkey ($cols);
}

sub p2h_font_to_font_size ($) {
    my ($font) = @_;
    my ($pt);

    if ($font->{family} eq 'Times'
	|| $font->{family} eq 'Helvetica'
	|| $font->{family} eq 'Courier'
	|| $font->{family} eq 'Symbol') {
	$pt = ($font->{size} + 3) / $zoom;
    } else {
	print STDERR "$banal_filename: Error: Unknown font family.\n";
#	print Dumper ($font);
	$pt = 0;
    }

    return $pt;
}

sub p2h_font_bug ($) {
    my ($doc) = @_;

    return 1 if ($doc->{pagespec}->{bodyfont} <= 0);
    return 0;
}

sub p2h_serious_font_bug ($) {
    my ($doc) = @_;

    return 0 if (!p2h_font_bug ($doc));
    return 1 if ($doc->{textbb}->{width} == 0 ||
		 $doc->{textbb}->{height} == 0);
    return 0;
}

sub report_verbose ($) {
    my ($doc) = @_;
    my ($page) = $doc->{pages}->{1};

    print $file, "\n";
    if (p2h_font_bug ($doc)) {
	print STDERR $file, "\n";
	print STDERR "$banal_filename: Error: pdftohtml encountered font problems...some info likely bogus.\n";
    }
    printf ("Paper size: %.2fin x %.2fin\n", $doc->{pagespec}->{paperbb}->{width}, $doc->{pagespec}->{paperbb}->{height});
    printf ("Text region: %.2fin x %.2fin\n", $doc->{textbb}->{width},
	    $doc->{textbb}->{height});
    printf ("Margins: %.2fin x %.2fin x %.2fin x %.2fin (l/r/t/b)\n",
	    $doc->{textbb}->{left},
	    $doc->{textbb}->{rmarg},
	    $doc->{textbb}->{top},
	    $doc->{textbb}->{bmarg});
    printf ("Body font size: %.2fpt", $doc->{pagespec}->{bodyfont});
    if (p2h_font_bug ($doc)) {
	print " (bogus)";
    }
    print "\n";
    printf ("Leading: %.1fpt\n", $doc->{pagespec}->{lead});
    print "Columns: ", $page->{pagespec}->{ncols}, "\n";
    print "Pages: ", $doc->{npages}, "\n";
    print "App: ", $doc->{app}, "\n";

    print "\n";
    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};

	print "Page $page->{num}:\n";
	printf ("  text region: %.2fin x %.2fin\n", $page->{pagespec}->{textbb}->{width}, $page->{pagespec}->{textbb}->{height});

	$left_i = $page->{pagespec}->{textbb}->{left};
	$right_i = $page->{pagespec}->{paperbb}->{width} - 
	    ($left_i + $page->{pagespec}->{textbb}->{width});
	$top_i = $page->{pagespec}->{textbb}->{top};
	$bot_i = $page->{pagespec}->{paperbb}->{height} -
	    ($top_i + $page->{pagespec}->{textbb}->{height});
	printf ("  margins: %.2fin x %.2fin x %.2fin x %.2fin (l/r/t/b)\n", 
		$left_i, $right_i, $top_i, $bot_i);

	printf ("  body font: %gpt (id %d)\n", $page->{pagespec}->{bodyfont},
		$page->{pagedata}->{bodyfont}->{id});
	printf ("  leading: %gpt\n", $page->{pagespec}->{lead});
	printf ("  columns: %d\n", $page->{pagespec}->{ncols});
	print   "  type: ", $page->{pagespec}->{type}, "\n";

	$density = $page->{pagespec}->{density};
	printf ("  density: %d\n", $density);
    }
}

sub report_stats ($) {
    my ($doc) = @_;
    my ($page) = $doc->{pages}->{1};

    if (p2h_serious_font_bug ($doc)) {
	print STDERR "$banal_filename: Error: pdftohtml encountered font problems...skipping.\n";
	return;
    }

    if (p2h_font_bug ($doc)) {
	print STDERR "$banal_filename: Warning: pdftohtml encountered font problems...some info likely bogus.\n";
    }

    printf ("$file\t%.2fx%.2f\t%.2fx%.2f\t%.2fx%.2fx%.2fx%.2f\t%d\t%.1f\t%d\t%d\t%s\n",
	    # page width x height
	    $doc->{pagespec}->{paperbb}->{width}, 
	    $doc->{pagespec}->{paperbb}->{height},
	    # text region width x height
	    $doc->{textbb}->{width},
	    $doc->{textbb}->{height},
	    # margins left x right x top x bottom
	    $doc->{textbb}->{left},
	    $doc->{textbb}->{rmarg},
	    $doc->{textbb}->{top},
	    $doc->{textbb}->{bmarg},
	    # body font
	    $doc->{pagespec}->{bodyfont},
	    # leading
	    $doc->{pagespec}->{lead},
	    # columns
	    $doc->{pagespec}->{ncols},
	    # pages
	    $doc->{npages},
	    # app
	    $doc->{app},
	    );
}

sub judge_paper_size ($$) {
    my ($doc, $spec) = @_;
    my ($msg) = '';
    my ($w, $h);

    $w = $doc->{pagespec}->{paperbb}->{width};
    $h = $doc->{pagespec}->{paperbb}->{height};
    if ($spec->{paper} eq 'letter') {
	$paperw = 8.5;
	$paperh = 11;
    } elsif ($spec->{paper} eq 'A4') {
	$paperw = 8.26;
	$paperh = 11.69;
    }

    unless (((($paperw - $banal_text_fudge) < $w) &&
	     (($paperw + $banal_text_fudge) > $w)) &&
	    ((($paperh - $banal_text_fudge) < $h) &&
	     (($paperh + $banal_text_fudge) > $h))) {
	$msg = sprintf ("Paper size: %.2f x %.2f is not $spec->{paper} size\n",
			$w, $h);
    }

    return $msg;
}

sub judge_page_count ($$) {
    my ($doc, $spec) = @_;
    my ($msg) = '';

    if ($doc->{npages} > $spec->{pages}) {
	$msg = sprintf ("Pages: too many pages %d (max %d)\n",
			$doc->{npages}, $spec->{pages});
    } elsif ($spec->{min_pages} &&
	     ($doc->{npages} < $spec->{min_pages})) {
	$msg = sprintf ("Pages: too few pages %d (min %d)\n",
			$doc->{npages}, $spec->{min_pages});
    }

    return $msg;
}

sub judge_body_font ($$) {
    my ($doc, $spec) = @_;
    my ($msg) = '';
    my ($i, $font);

    if (p2h_font_bug ($doc)) {
	$msg .= "Font: Cannot judge, no font info derived from pdf\n";
	return $msg;
    }

    if ($doc->{pagespec}->{bodyfont} < $spec->{font}) {
	$msg .= sprintf ("Font: body font too small %dpt (min %dpt)\n",
			 $doc->{pagespec}->{bodyfont}, $spec->{font});
    }
    return $msg if (1);

    # largest occuring bod
    # skip font on last page...typically smaller bibliography font
    for $i (1..($doc->{npages} - 1)) {
	$page = $doc->{pages}->{$i};

	# ignore pages with sparse text.
	# crude, but tough to use as a loophole.
	next if ($page->{pagespec}->{density} < $banal_min_density);

	$fonts->{$page->{pagespec}->{bodyfont}}++;
    }

    $bodyfont = modevalkey ($fonts);
#    next unless ($spec->{font} >= $bodyfont);

    return $msg;
}

sub judge_leading ($$) {
    my ($doc, $spec) = @_;
    my ($msg) = '';
    my ($lead);

    $lead = $doc->{pagespec}->{lead};
    if (($spec->{lead} - 0.1) > $lead) {
	$msg .= sprintf ("Leading: too small %.1fpt (min %.1fpt) using %s\n",
			 $lead, $spec->{lead}, $doc->{app});
    }
}

sub judge_columns ($$) {
    my ($doc, $spec) = @_;
    my ($msg) = '';
    my ($i, $page);

    # should add a 'strict' option
    if ($doc->{ncols} > $spec->{cols}) {
	$msg = sprintf ("Columns: found %d columns, expecting %d\n",
			$doc->{ncols}, $spec->{cols});
    }

    return $msg if (1);

    # skip last page
    for $i (1..($doc->{npages} - 1)) {
	$page = $doc->{pages}->{$i};

	next if ($page->{pagespec}->{density} < $banal_min_density);

	next unless ($spec->{cols} != $page->{pagespec}->{ncols});

	$msg = sprintf ("Columns: found %d columns, expecting %d\n",
			$page->{pagespec}->{ncols}, $spec->{cols});
	last;
    }

    return $msg;
}

sub judge_text_region ($$) {
    my ($doc, $spec) = @_;
    my ($wmsg, $hmsg) = ('', '');
    my ($i, $page);
    my ($width, $height, $width_fail, $height_fail);

    $width_fail = 0;
    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};

	# ignore pages without much text
	next if ($page->{pagespec}->{density} < $banal_min_density);

	$width = $page->{pagespec}->{textbb}->{width};
	next unless ($spec->{width} &&
		     ($width > ($spec->{width} + $spec->{fudge})));
	$width_fail++;
	
	$wmsg = sprintf ("Width: text too wide %.2fin (max %.2fin)\n",
			 $width, $spec->{width});
    }

    # if a small number of pages fail the width spec, it is likely
    # due to tables or figures extending into the margin.
    # only check on reasonably long docs.
    if ($doc->{npages} > (($banal_judge_min_fail_pages - 1) * 2)) {
	if ($width_fail < $banal_judge_min_fail_pages) {
	    $wmsg = '';
	}
    }


    $height_fail = 0;
    for $i (1..$doc->{npages}) {
	$page = $doc->{pages}->{$i};

	next if ($page->{pagespec}->{density} < $banal_min_density);

	$height = $page->{pagespec}->{textbb}->{height};
	next unless ($spec->{height} && 
		     ($height > ($spec->{height} + $spec->{fudge})));
	$height_fail++;

	$hmsg = sprintf ("Height: text too high %.2fin (max %.2fin)\n",
			 $height, $spec->{height});
    }

    # if a small number of pages fail the height spec, it is likely
    # due to tables or figures extending into the margin.
    # only check on reasonably long docs.
    if ($doc->{npages} > (($banal_judge_min_fail_pages - 1) * 2)) {
	if ($height_fail < $banal_judge_min_fail_pages) {
	    $hmsg = '';
	}
    }

#    $hmsg .= sprintf ("Fail: width $width_fail height $height_fail\n");

    return $wmsg . $hmsg;
}

sub pass_judgement ($$) {
    my ($doc, $spec) = @_;
    my ($page);
    my ($msg) = '';
    my ($err);

    if (p2h_serious_font_bug ($doc)) {
	print STDERR "$banal_filename: Error: pdftohtml encountered font problems...skipping.\n";
	return;
    }

    $msg .= judge_paper_size ($doc, $spec) if ($spec->{paper});
    $msg .= judge_page_count ($doc, $spec) if ($spec->{pages});
    $msg .= judge_body_font ($doc, $spec) if ($spec->{font});
    $msg .= judge_leading ($doc, $spec) if ($spec->{lead});
    $msg .= judge_columns ($doc, $spec) if ($spec->{cols});
    $msg .= judge_text_region ($doc, $spec) if ($spec->{width} || $spec->{height});

    return if (!$msg);
    
    if ($format eq 'list') {
	chop $msg;         # remove trailing newline
	$msg =~ s/\n/,/g;  # convert newlines to commas
	print basename ($file), ",$msg\n";
    } else {
	$msg =~ s/^(.)/  $1/mg;  # indent
	print $file, ":\n";
	print $msg;
    }

    if ($sc11_user_feedback) {
	if ($doc->{app} eq 'word') {
	    print "\n", $sc11_word_msg, "\n";
	} elsif ($doc->{app} eq 'tex') {
	    print "\n", $sc11_tex_msg, "\n";
	}
    }
}

sub parse_p2h_fonts ($$) {
    my ($line, $page) = @_;
    my (%fonts, $font, $fontid);

    while (1) {
#	print "p2h_font: $line";
	return $line if ($line =~ /<\/page>/);

	last unless ($line =~ /<fontspec id=\"(\d+)\" size=\"([-]*\d+)\" family=\"([A-Za-z0-9]+)\" color=\"(\#[a-fA-F0-9]+)\"\/>/);

	$font = { id => $1, size => $2, family => $3, color => $4 };
	$fontid = "$3//$2//$4";
	if (exists $fonts{$fontid}) {
	    $font->{id} = $fonts{$fontid};
	} else {
	    $fonts{$fontid} = $1;
	}
	$page->{doc}->{fonts}{$1} = $font;

	$line = <FILE>;
    }

    return $line;
}

sub update_segdata ($$$) {
    my ($page, $segdata, $seg) = @_;
    my ($top, $left, $width, $height, $font, $lead) = @$seg;
    my ($bottom) = $top + $height;
    my ($right) = $left + $width;
    my ($pagew) = $page->{pagedata}->{pagebb}->{width};

    $segdata->{widths}{$width}++ if ($width > $p2h_per_inch);
    $segdata->{lefts}{$left}++ if ($left < ($pagew / 3));
    $segdata->{rights}{$right}++ if ($right > ($pagew / 3));
    $segdata->{tops}{$top}++ if ($width > $p2h_per_inch);
    $segdata->{bots}{$bottom}++ if ($width > $p2h_per_inch);
#    $segdata->{leads}{$lead}++ if ($lead > 0 && $width > $p2h_per_inch);
    $segdata->{leads}{$lead}++ if ($lead > 0);

    # count number of segments in a given font size, weighted by the
    # width of the segment.  the font with the greatest weight
    # will be the body font.

    $segdata->{byfont}{$font} += $width;
}

sub check_p2h_error ($) {
    my ($line) = @_;

    # check for pdftohtml error strings embedded in output
    return 1 if ($line =~ /^stroke seems to be a pattern/);

    return 0;
}

sub parse_p2h_text ($$) {
    my ($line, $page) = @_;
    my ($top, $bottom, $left, $right, $width, $height, $font);
    my ($text, $lead, $prevheight);

    $segs_all = {};
    $segs_byfont = {};

    $prevheight = 0;

    while (1) {
#	next if (check_p2h_error ($line));

	unless ($line =~ /<text top=\"(-?\d+)\" left=\"(-?\d+)\" width=\"(-?\d+)\" height=\"(-?\d+)\" font=\"(-?\d+)\"/) {
	    # if we didn't match a <text>, then it should be an end of page
	    unless ($line =~ /<\/page>/) {
		if ($debug_parse) {
		    print "$banal_filename: Curious, expecting a </page> but found:\n";
		    print $line;
		}
	    }
	    last;
	}

	$height = $1;
	if ($prevheight < $height) {
	    $lead = $height - $prevheight;
	} else {
	    $lead = -1;
	}
	$prevheight = $height;

	@seginfo = ($1, $2, $3, $4, $5, $lead);
	if (($font = $page->{doc}->{fonts}{$5})) {
	    $seginfo[4] = $font->{id};
	}

	# sanity check the data somewhat...text from embedded figures
	# can produce surprising values
	if ($1 < 0 || $2 < 0 ||
	    ($1 > $page->{pagedata}->{pagebb}->{height}) ||
	    ($2 > $page->{pagedata}->{pagebb}->{width})) {
	    $line = <FILE>;
	    next;
	}

	$nsegs++;

	$segs_byfont->{$seginfo[4]} = {}
	   unless (defined $segs_byfont->{$seginfo[4]});
	$byfont = $segs_byfont->{$seginfo[4]};
	update_segdata ($page, $byfont, \@seginfo);
	$segs_byfont{$seginfo[4]} = $byfont;
	update_segdata ($page, $segs_all, \@seginfo);

	# embedded newlines will split <text>...</text> across multiple lines
	if ($line !~ /<\/text>/) {
	    while ($line = <FILE>) {
		print "$banal_filename: skipping: $line" if ($debug_parse);
		last if ($line  =~/<\/text>/);
	    }
	}

	$line = <FILE>;
    }


    $page->{pagedata}->{nsegs} = $nsegs;
    $page->{pagedata}->{segdata} = $segs_all;
    $page->{pagedata}->{segdata_byfont} = $segs_byfont;

    calc_page_body_font ($page);
    calc_page_leading ($page);
    calc_page_density ($page);
    calc_page_text_region ($page, $segs_all);
    calc_page_columns ($page);
}

sub parse_p2h_page ($) {
    my ($doc) = @_;

    # assume we've just read the header
    $line = <FILE>;

    # skip any error strings embedded between pages
    while (check_p2h_error ($line)) {
	print "$banal_filename: skipping p2h error string: $line" if ($debug_parse);
	$line = <FILE>;
    }

    unless ($line =~ /<page number=\"(\d+)\" position=\"([A-Za-z0-9]+\") top=\"(\d+)\" left=\"(\d+)\" height=\"(\d+)\" width=\"(\d+)\"/) {
	return '' if ($line =~ /<\/pdf2xml/);
	print "$banal_filename: Error: \"<page ...\" node expected for page ", $doc->{npages} + 1, "\n";
	print "-> '$line'";
	return '';
    }

    # initialize page data structures
    $pagebb = {
	top => $3,
	left => $4,
	height => $5,
	width => $6,
    };

    $paperbb = {
	top => $3 / $p2h_per_inch,
   	left => $4 / $p2h_per_inch,
    	height => $5 / $p2h_per_inch,
	width => $6 / $p2h_per_inch,
    };

    $page = {
	doc => $doc,
	num => $1,
	pagedata => {
	    pagebb => $pagebb,
	},
	pagespec => {
	    paperbb => $paperbb,
	},
    };

    # check for optional fontspecs at start of page
    $line = <FILE>;
    if ($line =~ /<fontspec/) {
	$line = parse_p2h_fonts ($line, $page);
    } elsif ($debug_parse) {
	print "$banal_filename: Curious, no fontspec on page, found:\n";
	print "$line";
    }


    # process text segments
    if ($line =~ /<text/) {
	parse_p2h_text ($line, $page);
    } elsif ($debug_parse) {
	print "$banal_filename: Curious, empty page $page->{num}, found:\n";
	print "$line";
    }

    return $page;
}

sub parse_p2h_header ($) {
    my ($doc) = @_;

    while (<FILE>) {
	return 1 if (/<pdf2xml>/);
    }
    return 0;
}

sub merge_page ($$) {
    my ($doc, $page) = @_;

    $doc->{npages}++;
    $doc->{pages}->{$page->{num}} = $page;

    # initialize doc spec with first page spec
    if ($page->{num} == 1) {
	$doc->{pagespec}->{paperbb} = $page->{pagespec}->{paperbb};
	$doc->{pagespec}->{textbb} = $page->{pagespec}->{textbb};
	$doc->{pagespec}->{bodyfont} = $page->{pagespec}->{bodyfont};
	$doc->{pagespec}->{ncols} = $page->{pagespec}->{ncols};
	return;
    }
}

sub banal_get_spec () {
    my ($s) = {};

    return $s unless (defined $judge);

    if (defined $testspec) {
	$s->{paper} = 'letter';
	$s->{pages} = 14;
	$s->{font} = 10;
	$s->{lead} = 12.0;
	$s->{cols} = 2;
	$s->{width} = 6.5;
	$s->{height} = 9;
	$s->{fudge} = $banal_text_fudge;
    }

    if (defined $paper) {
	if ($paper ne 'letter' && $paper ne 'A4') {
	    die ("$banal_filename: Error: Unknown paper type '$paper'.\n");
	}
	$s->{paper} = $paper;
    }
    $s->{pages} = $pages if (defined $pages);
    $s->{font} = $font if (defined $font);
    $s->{lead} = $leading if (defined $leading);
    $s->{cols} = $cols if (defined $cols);
    if (defined $width) {
	$s->{width} = $width;
	$s->{fudge} = $banal_text_fudge;
    }
    if (defined $height) {
	$s->{height} = $height;
	$s->{fudge} = $banal_text_fudge;
    }
    if (defined $fudge) {
	$s->{fudge} = $fudge;
    }
    return $s;
}

sub banal_report_spec ($) {
    my ($spec) = @_;

    print "Judging: ";
    print "$spec->{paper}, " if ($spec->{paper});
    print "$spec->{width}in x $spec->{height}in (~$spec->{fudge}), " if ($spec->{width} || $spec->{height});
    print "$spec->{font}pt font, " if ($spec->{font});
    print "$spec->{lead}pt leading, " if ($spec->{lead});
    print "$spec->{cols} cols, " if ($spec->{cols});
    print "$spec->{pages} pages" if ($spec->{pages});
    print "\n";
    print "-   -   -   -   -   -   -   -   -   -   -   -   -   -   -   -   -   -   \n";
}

sub banal_file ($$) {
    my ($file, $spec) = @_;

    # initialize doc data structure
    $doc = {
	width => 0,
	height => 0,
	npages => 0,
	ncols => 0,
	fonts => {},
	pages => {},
	textbb => {},
        app => '',
	fullpath => '',
	filename => '',
    };

    $doc->{fullpath} = $file;
    $banal_fullpath = $file;
    $doc->{filename} = basename ($file);
    $banal_filename = basename ($file);

    if (!parse_p2h_header ($doc)) {
	print STDERR "$banal_filename: Error: No pdftohtml output...corrupted pdf file?\n";
	return;
    }

    calc_doc_app ($doc);

    while ($page = parse_p2h_page ($doc)) {
	merge_page ($doc, $page);
    }

    calc_doc_body_font ($doc);
    calc_doc_leading ($doc);
    calc_doc_text_region ($doc);
    calc_doc_page_types ($doc);
    calc_doc_columns ($doc);

    if (defined $judge) {
	pass_judgement ($doc, $spec);
    } elsif (defined $stats) {
	report_stats ($doc);
    } else {
	report_verbose ($doc)
    }
}

sub banal_open_input ($) {
    my ($fname) = @_;
    my ($base, $ext, $cmd);

    if ($fname =~ /(.+)\.(.+)/) {
	($base, $ext) = ($1, $2);
    } else {
	print STDERR "$fname: Error: Unable to determine file type from extension.\n";
	return 0;
    }

    # 2>&1
    if ($ext =~ /[pP][dD][fF]/) {
	$zoomarg = ($zoom == 1 ? "" : "-zoom $zoom");
	$cmd = "$pdftohtml -stdout -enc UTF-8 -xml $zoomarg $fname 2>/dev/null |";
	print "$cmd\n" if ($debug_pdftohtml);

	unless (open (FILE, $cmd)) {
	    print STDERR "$fname: Error: Failed to open file.\n";
	    return 0;
	}
    } elsif ($ext =~ /[xX][mM][lL]/) {
	unless (open (FILE, "$fname")) {
	    print STDERR "$fname: Error: Failed to open file.\n";
	    return 0;
	}
    } else {
	print STDERR "$fname: Error: Failed to open file.\n";
	return 0;
    }
    binmode (FILE, ":utf8");

    return 1;
}

sub banal_config_p2h () {
    my ($major, $minor);

    unless (open (P2H, "$pdftohtml -v 2>&1 |")) {
	print STDERR "$fname: Error: Failed to run $pdftohtml.\n";
	return 0;
    }
    while (<P2H>) {
	next unless (/pdftohtml version (\d+\.\d+)([a-z]*)/);
	$p2h_version = "$1$2";
	$major = $1;
	$minor = $2;
	print "version $major$minor\n";
	last;
    }
    close (P2H);

    if (($major >= 0.40) && $minor && (($minor cmp "c") >= 0)) {
	# configure for versions 0.40c and above
	$zoom = 10 if !defined ($zoom);
	# always need to specify a zoom value for 0.40c
	$zoom = 1.001 if ($zoom == 1);
    } else {
	$zoom = 3 if !defined ($zoom);
    }

    if ($leading_policy) {
	$banal_leading_policy = $leading_policy;
    } else {
	# use a default policy according to the zoom level we can use
	# at low zoom, interpolate
	if ($zoom >= 10) {
	    $banal_leading_policy = 'mode';
	} else {
	    $banal_leading_policy = 'interpolate';
	}
    }

    print "leading policy: $banal_leading_policy\n" if ($debug_leading);


    $p2h_per_inch = 72 * $zoom;
    $p2h_to_points = 72 / $p2h_per_inch;

    return 1;
}

sub banal_version () {
    print "Banal version $banal_version.\n";
    return 0;
}

sub main () {
    my ($spec);

    return banal_version () if (defined $version);

    usage if ($#ARGV < 0);

    $spec = banal_get_spec ();
    banal_report_spec ($spec) if (defined $judge);

    if (!banal_config_p2h ()) {
	return 1;
    }

    foreach $file (@ARGV) {
	# open input file into FILE
	next unless (banal_open_input ($file));
	banal_file ($file, $spec);
	close (FILE);
    }
    return 0;
}

exit (main ());

#
# 2012-2-18
#    (banal_config_p2h): always specify a zoom value with pdftohtml 0.40c
#
# 2011-1-25
#    (utf8revbin_undo): new function; a tool incorrectly reverses multibytes
#
# 2011-1-19
#    (check_p2h_error): skip 'stroke seems...' pdftohtml output that can
#    appear between page output.
#
# 2011-1-18
#    (parse_p2h_page, parse_p2h_text, parse_p2h_fonts): handle <text>
#    segments that span multiple lines from embedded newlines accurately.
#    handle optional <fontspecc> commands more gracefully.
#    (debug_parse): new flag.
#
# 2011-1-17
#    (update_segdata): fix reporting negative leadings.
#
# 2011-1-11
#    (utf8ascii_undo, utf8bin_undo, utf8hex_undo, calc_doc_app): new functions
#    for inferring the application used to create the document.
#    (report_verbose, report_stats, judge_leading): report doc application.
#    (debug_docapp): new flag.
#
# 2011-1-07
#    uniformly print filename in error messages.
# 
# 2010-12-31
#    (judge_format): new flag, option 'list' reports all violations
#    on a single line in CSV format.  default option 'lines' is original
#    behavior with one per line.
#

